Verification with Common Knowledge of Rationality for Graph Games

Realizability asks whether there exists a program satisfying its specification. In this problem, we assume that each agent has her own objective and behaves rationally to satisfy her objective. Traditionally, the rationality of agents is modeled by a Nash equilibrium (NE), where each agent has no incentive to change her strategy because she cannot satisfy her objective by changing her strategy alone. However, an NE is not always an appropriate notion for the rationality of agents because the condition of an NE is too strong; each agent is assumed to know strategies of the other agents completely. In this paper, we use an epistemic model to define common knowledge of rationality of all agents (CKR). We define the verification problem as a variant of the realizability problem, based on CKR, instead of NE. We then analyze the complexity of the verification problems for the class of positional strategies.

==> epistemic_model/kt5_example.tex <==
\begin{example}
    Let $1$ and $2$ be two players.
    There are three cards labeled $A$, $B$ and $C$ respectively.
    Player $1$ draws one card from them, then Player $2$ draws one card from the others.
    Both players know only the letter of the card they draw.
    Figure~\ref{fig:frame} shows a KT5 Kripke frame $(W,(R_p)_{p\in P})$
    expressing the knowledge of players where
    $P = \{ 1, 2\}$,
    $W = \{ AB, AC, BA, BC, CA, CB \}$,
    $R_1 = \{ (XY,XZ) \mid X,Y,Z \in \{ A,B,C \}, X\neq Y, X \neq Z \}$ and
    $R_2 = \{ (YX,ZX) \mid X,Y,Z \in \{ A,B,C \}, X\neq Y, X \neq Z \}$.
    \begin{figure}[t]
		\centering
		\begin{tikzpicture}[everynode/.style={circle,draw,minimum size=0.8cm},>=stealth]
            \node[everynode] (AB) at ({60}: 1.8) {$AB$};
            \node[everynode] (BA) at ({120}: 1.8) {$BA$};
            \node[everynode] (BC) at ({180}: 1.8) {$BC$};
            \node[everynode] (CA) at ({240}: 1.8) {$CA$};
            \node[everynode] (CB) at ({300}: 1.8) {$CB$};
            \node[everynode] (AC) at ({0}: 1.8) {$AC$};
            %self loop
            \draw[<->] (AB) to [loop above] node {$1,2$} (AB);
            \draw[<->] (BA) to [loop above] node {$1,2$} (BA);
            \draw[<->] (BC) to [loop left] node {$1,2$} (BC);
            \draw[<->] (AC) to [loop right] node {$1,2$} (AC);
            \draw[<->] (CA) to [loop below] node {$1,2$} (CA);
            \draw[<->] (CB) to [loop below] node {$1,2$} (CB);
            %
            \draw[<->] (AB) to[above right] node {$1$} (AC);
            \draw[<->] (BA) to[above left] node {$1$} (BC);
            \draw[<->] (CA) to[below] node {$1$} (CB);
            \draw[<->] (AB) to[above] node {$2$} (BA);
            \draw[<->] (BC) to[below left] node {$2$} (CA);
            \draw[<->] (AC) to[below right] node {$2$} (CB);
		\end{tikzpicture}
			\caption{KT5 Kripke frame expressing the knowledge of players in the three-card game}
			\label{fig:frame}
	\end{figure}
    The name of a world expresses which cards they drew.
    For example, the world $AB$ is the world such that Player $1$ draws the card $A$ and 
    Player $2$ draws the card $B$.
    Let $E = \{ AB, AC \}$ be the event such that Player $1$ draws the card $A$, and
    $F = \{ AB,AC,BA,BC \}$ be the event such that Player $1$ draws the card $A$ or $B$.
    %The event $\{ AB, AC \}$ is the set of worlds such that Player $1$ drew the card $A$.
    %Because $R_1(AB)\subseteq A1$, $AB \in \calK_p(\{ AB, AC \})$.
    %In both worlds $AB$ and $AC$, Player $1$ knows that she drew the card $A$
    Then, the event $\calK_1(E) = E$ is the event such that Player $1$ knows that she drew the card $A$.
    The event $\calMK(F) = \{ AC,BC \}$ is the event such that both players $1$ and $2$ know that 
    Player $1$ drew the card $A$ or $B$.
    Because $\calCK(W) = W$, the event $W$ is common knowledge in any world.
\end{example}
